ViM: Vision Middleware for Unified Downstream Transferring

Foundation models are pre-trained on massive data and transferred to downstream tasks via fine-tuning. This work presents Vision Middleware (ViM), a new learning paradigm that targets unified transferring from a single foundation model to a variety of downstream tasks. ViM consists of a zoo of lightweight plug-in modules, each of which is independently learned on a midstream dataset with a shared frozen backbone. Downstream tasks can then benefit from an adequate aggregation of the module zoo thanks to the rich knowledge inherited from midstream tasks. There are three major advantages of such a design. From the efficiency aspect, the upstream backbone can be trained only once and reused for all downstream tasks without tuning. From the scalability aspect, we can easily append additional modules to ViM with no influence on existing modules. From the performance aspect, ViM can include as many midstream tasks as possible, narrowing the task gap between upstream and downstream. Considering these benefits, we believe that ViM, which the community could maintain and develop together, would serve as a powerful tool to assist foundation models.

==> sections/6.ref.tex <==
{\small
\bibliographystyle{ieee_fullname}
\bibliography{ref}
}


==> tab/moe_k.tex <==
\begin{table}[htbp]
\caption{Ablation study on the $k$ of MoE under the ensemble and reparameterization (classification with ViM-joint tuning).}
\begin{tabular}{lccccc}
\toprule
method & $k=2$ & $k=4$ & $k=6$ & $k=8$ & $k=10$ \\
\midrule
Ens-MoE & 74.38 & 74.19 & 74.94 &  74.87 &\textbf{75.11} \\
Rep-MoE & 74.48 & 74.73 & 74.54 &  \textbf{74.77}   & 74.48 \\
\bottomrule
\end{tabular}
\label{tab:moe_k}
\end{table}
